SRA 2: Variational Autoencoder Self-Representation Alignment for Efficient Diffusion Training

Denoising-based diffusion transformers, despite their strong generation performance, suffer from inefficient training convergence. Existing methods addressing this issue, such as REPA (relying on external representation encoders) or SRA (requiring dual-model setups), inevitably incur heavy computational overhead during training due to external dependencies. To tackle these challenges, this paper proposes SRA 2, a lightweight intrinsic guidance framework for efficient diffusion training. SRA 2 leverages off-the-shelf pre-trained Variational Autoencoder (VAE) features: their reconstruction property ensures inherent encoding of visual priors like rich texture details, structural patterns, and basic semantic information. Specifically, SRA 2 aligns the intermediate latent features of diffusion transformers with VAE features via a lightweight projection layer, supervised by a feature alignment loss. This design accelerates training without extra representation encoders or dual-model maintenance, resulting in a simple yet effective pipeline. Extensive experiments demonstrate that SRA 2 improves both generation quality and training convergence speed compared to vanilla diffusion transformers, matches or outperforms state-of-the-art acceleration methods, and incurs merely 4% extra GFLOPs with zero additional cost for external guidance models.

==> tables/hyper_setting.tex <==
\begin{table}[t]
    \vspace{-1em}
    \centering
    \caption{\textbf{Default hyperparameter setup.} Unless otherwise specified, we use these hyperparameter sets for different models. In our component-wise analysis experiments, all settings remain unchanged except for those specified in Tab.1 of the main text.}
    % \vspace{0.3em}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l c c c}
        \toprule
         & SiT-B & SiT-L & SiT-XL \\
        \midrule
        \textbf{Architecture} \\
        Input dim. & 32$\times$32$\times$4 & 32$\times$32$\times$4 & 32$\times$32$\times$4 \\
        Patch size & 2 & 2 & 2 \\
        Num. layers & 12 & 24 & 28 \\
        Hidden dim. & 768 & 1024 & 1152 \\
        Num. heads & 12 & 16 & 16 \\ 
        \midrule
        \textbf{\name} \\
        Alignment blocks & $2$  & $8$ & $8$  \\
        Alignment timestep & $[0, 1]$ & $[0, 1]$ & $[0, 1]$  \\
        Objective & smooth-$\ell_1$ & smooth-$\ell_1$ & smooth-$\ell_1$ \\
        Using projection head & $\checkmark$ & $\checkmark$ & $\checkmark$  \\
        $\lambda$ & 1.0  & 1.0 & 1.0 \\
        \midrule
        \textbf{Optimization} \\
        Batch size & 256 & 256 & 256 \\ 
        Optimizer & AdamW & AdamW & AdamW  \\
        lr & 0.0001 & 0.0001 &  0.0001 \\
        $(\beta_1, \beta_2)$ & (0.9, 0.999) & (0.9, 0.999) & (0.9, 0.999) \\
        \midrule
        \textbf{Interpolants or Denoising} \\
        $\alpha_t$ & $1-t$ & $1-t$ & $1-t$ \\
        $\sigma_t$ & $t$ & $t$ & $t$ \\
        $w_t$ & $\sigma_t$ & $\sigma_t$ & $\sigma_t$\\
        Training objective & v-prediction & v-prediction & v-prediction \\
        Sampler & Euler-Maruyama & Euler-Maruyama & Euler-Maruyama  \\
        Sampling steps & 250 & 250 & 250 \\
        Guidance Scale& - & - & 1.8 (if used) \\
        \bottomrule
    \end{tabular}}
    \vspace{-0.5em}
    \label{tab:hyperparam}
\end{table}
